On the (k,l)-anonymity of networks via their $k$-metric antidimension

This work focuses on the (k,l)-anonymity of some networks as a measure of their privacy against active attacks. Two different types of networks are considered. The first one consists of graphs with a predetermined structure, namely cylinders, toruses, and $2$-dimensional Hamming graphs, whereas the second one is formed by randomly generated graphs. In order to evaluate the (k,l)-anonymity of the considered graphs, we have computed their k-metric antidimension. To this end, we have taken a combinatorial approach for the graphs with a predetermined structure, whereas for randomly generated graphs we have developed an integer programming formulation and computationally tested its implementation. The results of the combinatorial approach, as well as those from the implementations indicate that, according to the (k,l)-anonymity measure, only the 2-dimensional Hamming graphs and some general random dense graphs are achieving some higher privacy properties.

==> Sec-ILPv.tex <==
\section{Integer programming formulation for the $k$-MAD problem}\label{sect:k_ILP}

In this section we develop an integer programming formulation for finding the $k$-metric antidimension of a given graph $G$. Abusing slightly the notation, we also denote by $V=\{1, \dots, n\}$ the set of indices associated with the vertices of the graph in a natural way. The formulation, which is based on the definition of a $k$-ARS $S$, through the equivalence relation $\mathcal{R}_S$, is built over two sets of binary decision variables, one to determine the elements of the set $S$ and another one to determine the elements of the different classes.
The vertex classes are determined by subsets of vertices that jointly satisfy some compatibility conditions, and will be referred to as $Q$-\emph{subsets}. To avoid multiple representations of the same solution, each $Q$-subset has a unique representative, which is its lowest index vertex.


We define the following sets of decision variables:
\begin{align}
s_u & = 1 \qquad \text{ if and only if } u \in S, \qquad && \forall u\in V \nonumber \\
q_{uv} & = 1 \qquad\text{ if and only if } v\text{ is in the $Q$-subset with representative $u$} \qquad && \forall u,v\in V, v\geq u.\nonumber
\end{align}

The above decision variables determine vertex sets $S=\{u \in V: s_u=1\}$ of cardinality $|S|=\sum_{u \in V} s_u$, and $Q$-subsets $Q^u=\{v\in V: q_{uv}=1\}$. Since $q_{uu}=1$ indicates that $u$ is the lowest index vertex of a $Q$-subset, the actual number of classes determined by the solution is $\overline r=\sum_{u\in V}q_{uu}$.

The formulation is as follows.

\begin{align}
F\qquad\hspace{-0.3cm}\min \quad &  \sum_{u \in V} s_u  && \\
& \sum_{u\in V} s_{u}  \ge 1 && \label{2ineq:S-non-empty}\\
& s_u+\sum_{v\in V: v\leq u} q_{vu}  = 1 && u\in V\label{2ineq:partition}\\ 
& \sum_{v\in V: v> u} q_{uv}  \ge (k-1) q_{uu} && u \in V \label{2ineq:cardinality}\\ 
& s_u+\,q_{vw}  \leq 1  && u, v, w\in V,\, u\ne v,\, v<w,\, d_{uv}\ne d_{uw} \label{2ineq:incompatibility}\\        
& s_{v}+q_{uv}+\sum_{\substack{w\in V:w\ne u,\, w\ne v, \\ d_{uw}\ne d_{vw}}}s_w \geq q_{uu} \qquad && u,v\in V, v>u \label{2ineq:maximal}\\ 
& s_u\in\{0, 1\}, \, \forall u\in V; && q_{uv}\in\{0, 1\}, u, v \in V, v\geq u.
\end{align}

Let $\Omega$ denote the domain determined by the feasible solutions to $F$, {\em i.e.} $\Omega=\{(s, q): s\in\{0, 1\}^{n}, q \in\{0, 1\}^{n\choose 2} \text{ satisfy } \eqref{2ineq:S-non-empty}-\eqref{2ineq:maximal}\}$.

\begin{prop}\label{propo1}
Any feasible solution $(s, q)\in\Omega$ determines a $k$-{ARS}.
\end{prop}

\begin{proof}
Let $(s, q)\in\Omega$. Consider $S=\{u \in V:  s_u=1\}$ and the $Q$-subsets $Q^u=\{v\in V: q_{uv}=1\}$. Let us see that these $Q$-subsets are precisely the classes determined by the equivalence relation $\mathcal R_{S}$. To this end, we analyze the meaning of the constraints:
\begin{itemize}
\item Constraint \eqref{2ineq:S-non-empty} guarantees that the vertex set $S$ is non-empty. 
\item Constraints \eqref{2ineq:partition} ensure that we obtain a partition by imposing that each vertex $u \in V$ belongs either to set $S$ ($s_u=1$) or to some $Q$-subset, where the representative is either vertex $u$ or a vertex with a lower index. 
\item Constraints \eqref{2ineq:cardinality} guarantee that the cardinality of each $Q$-subset is at least $k$. Note that these constraints are only active when $u$ is the representative of some $Q$-subset ($q_{uu}=1$) and impose that, in such a case, the $Q$-subset associated with $u$ has at least $k-1$ additional elements. This guarantees that $|Q^u|\geq k$.
\item Constraints \eqref{2ineq:incompatibility} ensure that the $Q$-subsets are well defined so the pairs of vertices in each component satisfy the \emph{compatibility}  criterion, by imposing that no two vertices $v, w\in V$ with different distance to any vertex $u\in S$ may belong to the same $Q$-subset. When $w=u$ these constraints impose that the $Q$-sets only contain vertices that are not in $S$. 
\item The role of Constraints~\eqref{2ineq:maximal} is to guarantee that the obtained $Q$-subsets are precisely the classes determined by the equivalence relation $\mathcal R_{S}$. In other words, they guarantee that all the vertices in the same equivalence class of $\mathcal R_{S}$ are assigned to the same $Q$-subset. Note that Constraints \eqref{2ineq:incompatibility} do not guarantee this condition since, in principle, two vertices of the same equivalence class of $\mathcal R_{S}$ could be assigned to different $Q$-subsets.
Observe that the constraint \eqref{2ineq:maximal} associated with a given vertex pair $u,v\in V, u< v$ is only active when $u$ is the representative of $Q$-subset $Q^u$. In such a case, the constraint holds trivially if $v$ belongs either to $S$ or to $Q^u$. Otherwise, the constraint imposes that there exists some vertex $w\in S$ such  that $d_{uw}\ne d_{vw}$. That is, $u$ and $v$ do not belong to the same the equivalence of $\mathcal R_{S}$.\\
\end{itemize}
The conclusion of the above analysis is that any feasible solution $(s, q)\in\Omega$ determines a $k$-ARS and its objective function value $|S|=\sum_{u \in V}  s_u$.
\end{proof}

Below we see that the reverse of the above result also holds. In particular

\begin{prop}\label{propo2}
Any $k$-ARS $S\subset V$, $\{Z^r\}_{r\in R}$ can be associated with a solution in $(s, q)\in\Omega$.
\end{prop}


\begin{proof}
Let $S\subset V$, $\{Z^r\}_{r\in R}$ be a given $k$-ARS. Consider the following solution $(s, q)$:
  \begin{itemize}\item $s_u=1$ if and only if $u\in S$.
  \item $q_{uv}=1$ if and only if $u,v\in Z^r$, $u<v$, and $ q_{u^r, u^r}=1$ with $u^r=\min\{u: u\in Z^r\}$, $r\in R$. \\
  (that is, $Q^{u^r}=Z^r$, $r\in R$).
\end{itemize}
Let us see that $(s, q)\in \Omega$:
\begin{itemize}
\item $S\ne\emptyset$ implies that there exists $u\in S$, and thus   \eqref{2ineq:S-non-empty} holds.
    \item Since $S\cup\{ Z^r\}_{r\in R}$ determines a partition of $V$, by definition, $(s, q)$ satisfies \eqref{2ineq:partition}. 
\item Since $S\subset V$, $\{Z^r\}_{r\in R}$ is a $k$-ARS, for any class $r\in R$ it holds that for any pair of vertices $v,w\in V$ such that $d_{uv}\ne d_{uw}$ for some $u\in S$, then $v$ and $w$ cannot both belong to the same equivalence class $Z^r= Q^{u^r}$, $r\in R$. In other words, if $s_u=1$, then $q_{v,w}=0$ for all $r\in R$. Hence, $(s, q)$ also satisfies constraints \eqref{2ineq:incompatibility}.
\item Since $|Z^r|\geq k$, for all $r\in R$, $|Z^r\setminus \{u^r\}|=|Q^{u^r}\setminus \{u^r\}|\geq k-1$, for all $r\in R$. Hence the constraints \eqref{2ineq:cardinality}, which are only activated for the vertices $u^r$, $r\in R$,  are satisfied by  $(s, q)$.
\end{itemize}
\end{proof}

\begin{rem}
Note that Constraints \eqref{2ineq:S-non-empty} in formulation $F$ impose that the vertex set  $S$ induced by the solution is non-empty. This means that the optimal value of $F$ will be $\adim_k(G)$, when a $k$-ARS exists. However, when no $k$-ARS 
exists for a given value of $k$, then the formulation $F$ will have no feasible solution.
\end{rem}
As a consequence of the above analysis, we deduce the following statement.

\begin{cor}
$F$ is a valid formulation for \eqref{$k$-MAD Problem} on a given graph $G=(V, E)$. 
When $F$ is feasible, then its optimal value determines $\adim_k(G)$. Otherwise, if $F$ is infeasible, then no $k$-ARS exists.
\end{cor}


\begin{proof}
As a consequence of Propositions \ref{propo1} and \ref{propo2}, there is a one-to-one correspondence between $k$-ARS and feasible solutions in $\Omega$. 
Moreover, the  objective function value of feasible solution $(s, q)\in\Omega$, is $|S|=\sum_{u \in V}  s_u$. 
Therefore, since $F$ is a minimization problem, any optimal solution to $F$ will determine a $k$-ARS and its objective function value $\adim_k(G)$.
\end{proof}


The formulation $F$ above has $n+ {n \choose 2}$ binary decision variables, and a number of constraints $\mathcal{O}\left(1+2n+\left(n+1\right){n \choose 2}\right)$.
In particular, the number of Constraints~\eqref{2ineq:incompatibility} is $(n-2){n \choose 2}$. Since this number can be too big as the number of vertices of the graph increases, we develop an aggregated version of this set of constraints, namely:
\begin{align}
\sum_{u\in V: d_{uv}\ne d_{uw}}s_u+ n\,q_{vw} & \leq n && \forall v,w \in V, v\geq w, \label{2ineq:Classes_agg}
\end{align}
which takes into account that in any feasible solution $S$, for any pair $v,w\in V$, $v< w$,  it holds that $\sum_{u\in V: d_{uv}\ne d_{uw}}s_u\le \sum_{u\in V}s_u\le n$. 
Since the right hand side of Constraints \eqref{2ineq:Classes_agg} is precisely $n$, the constraint associated with a given pair of vertices $v, w$ prevents that both vertices belong to the same $Q$-set when there exists some vertex $u\in S$ such that $d_{uv}\ne d_{uw}$. 
Hence by substituting Constraints \eqref{2ineq:incompatibility} with Constraints \eqref{2ineq:Classes_agg} we obtain an alternative valid formulation for \eqref{$k$-MAD Problem}, which will be referred to as $F^{A}$.
Note that the number of Constraints~\eqref{2ineq:Classes_agg} is ${n^2 \choose 2}$, which is one order of magnitude less than that of Constraints \eqref{2ineq:incompatibility}.



==> sec-bibliov.tex <==
\bibliographystyle{abbrv}
\begin{thebibliography}{10}

\bibitem{Cangalovic-2018} \v{C}angalovi\'c, M., Kova\v{c}evi\'c-Vuj\v{c}i\'c, V., and Kratica, J. (2018). $k$-metric antidimension of wheels and grid graphs. Proceeding of the ``XIII Balkan Conference on Operational Research'', Belgrade, Serbia. ISBN: 978-86-80593-64-7.

\bibitem{Chatterjee-2019} Chatterjee, T., DasGupta, B., Mobasheri, N., Srinivasan, V., and Yero, I. G. (2019). On the computational complexities of three problems related to a privacy measure for large networks under active attack, Theoretical Computer Science 775, 53--67.

\bibitem{DasGupta-2019} DasGupta, B., Mobasheri, N., and Yero, I. G. (2019). On analyzing and evaluating privacy measures for social networks under active attack Information Sciences 473, 87--100.

\bibitem{Hammack-2011} Hammack, R. H., Imrich, W., and Klav\v{z}ar, S. (2011). Handbook of product graphs (Vol. 2). Boca Raton: CRC press. New York.

\bibitem{Kuziak-2021} Kuziak, D., and Yero, I. G. (2021). Metric dimension related parameters in graphs: A survey on combinatorial, computational and applied results. arXiv preprint arXiv:2107.04877.

\bibitem{Kratica-2019} Kratica, J., Kova\v{c}evi\v{c}-Vuj\v{c}i\'c, V., and \v{C}angalovi\'c, M. (2019). $k$-metric antidimension of some generalized Petersen graphs, Filomat 33(13), 4085--4093.

\bibitem{Mauw-2019} Mauw, S., Ram\'irez-Cruz, Y., and Trujillo-Rasua, R. (2019). Conditional adjacency anonymity in social graphs under active attacks, Knowledge and Information Systems 61(1), 485--511.

\bibitem{Mauw-2018} Mauw, S., Ram\'irez-Cruz, Y., and Trujillo-Rasua, R. (2018). Anonymising social graphs in the presence of active attackers. Transaction on Data Privacy 11(2), 169--198.

\bibitem{Tang-2021} Tang, J. H., Noreen, T., Salman, M., Rehman, M. U., and Liu, J. B. (2021). $(k,\ell)$-anonymity in wheel-related social graphs measured on the base of $k$-metric antidimension, Journal of Mathematics, vol 2021, Article ID 8038253.

\bibitem{Trujillo-Rasua-2016-a} Trujillo-Rasua, R., and Yero, I. G. (2016). Characterizing $1$-metric antidimensional trees and unicyclic graphs, Computer Journal 59(8), 1264--1273.

\bibitem{Trujillo-Rasua-2016} Trujillo-Ras\'ua, R., and Yero, I. G. (2016). $k$-metric antidimension: A privacy measure for social graphs, Information Sciences 328, 403--417.

\bibitem{Xpress} Xpress.
\newblock Fico$^{\tiny{\mbox{\textregistered}}}$ xpress solver.
\newblock \url{https://www.fico.com/es/products/fico-xpress-solver}.
\newblock Accessed: 2020-11-10.

\bibitem{Zhang-2017} Zhang, C., and Gao, Y. (2017). On the complexity of $k$-metric antidimension problem and the size of $k$-metric antiresolving sets in random graphs. In International Computing and Combinatorics Conference (pp. 555--567). Springer, Cham.

\end{thebibliography}
